Learning to Help in Multi-Class Settings

Deploying complex machine learning models on resource-constrained devices is challenging due to limited computational power, memory, and model retrainability. To address these limitations, a hybrid system can be established by augmenting the local model with a server-side model, where samples are selectively deferred by a rejector and then sent to the server for processing. The hybrid system enables efficient use of computational resources while minimizing the overhead associated with server usage. The recently proposed Learning to Help (L2H) model trains a server model given a fixed local (client) model, differing from the Learning to Defer (L2D) framework, which trains the client for a fixed (expert) server. In both L2D and L2H, the training includes learning a rejector at the client to determine when to query the server. In this work, we extend the L2H model from binary to multi-class classification problems and demonstrate its applicability in a number of different scenarios of practical interest in which access to the server may be limited by cost, availability, or policy. We derive a stage-switching surrogate loss function that is differentiable, convex, and consistent with the Bayes rule corresponding to the 0-1 loss for the L2H model. Experiments show that our proposed methods offer an efficient and practical solution for multi-class classification in resource-constrained environments.

==> secs/consistency.tex <==
\section{Consistency and Calibration}

\subsection{Classification consistency}
The minimizer works as the same as Bayes while the function family is all measurable functions.
\subsection{F-conssitency}
from \cite{verma2022calibrated} paper appendix.
\subsection{F-calibration}
\subsection{l-consistency}

\subsection{M,R consistency}

\subsection{H-consistency}
Used by series papers from Anqi Mao.


==> secs/multi_class_surrogate_loss.tex <==
\section{Surrogate Loss Function}
Seems like for multi class classification, 
we can't use just a single function to determine the label( like in binary, $f>0$ or $f<+0$ represent different labels.). Usually, we should define something like
\begin{align}
    \arg \max_{i} g_i(x)
\end{align}
where $g_i(x)$ represents "score function" for each class.
\subsection{Softmax based class}
\subsubsection{Cross Entropy}
This method is from \cite{mozannar2020consistent}
The surrogate loss is 
\begin{align}
    L_{C E}(h, r, x, y, m)=-\log \left(\frac{\exp \left(g_y(x)\right)}{\sum_{y^{\prime} \in \mathcal{Y} \cup \perp} \exp \left(g_{y^{\prime}}(x)\right)}\right)-\mathbb{I}_{m=y} \log \left(\frac{\exp \left(g_{\perp}(x)\right)}{\sum_{y^{\prime} \in \mathcal{Y} \cup \perp} \exp \left(g_{y^{\prime}}(x)\right)}\right)
\end{align}
where $m$ is the expert.
Proof of consistency: since it's convex, calculate the derivation and find the minimizer. Then show that minimizer is the same as Bayes in some ways.
\subsubsection{Realizable Cross Entropy}
This method is from \cite{mozannar2023should}  
\begin{align}
    L_{R S}(\mathbf{g}, \cdot)=-2 \log \left(\frac{\exp \left(g_y(x)\right)+\mathbb{I}_{h=y} \exp \left(g_{\perp}(x)\right)}{\sum_{y^{\prime} \in \mathcal{Y} \cup \perp} \exp \left(g_{y^{\prime}}(x)\right)}\right)
\end{align}
where $h$ denotes the fixed human predictor.

Define the another consistency (M, R)-consistent surrogate. Then use Sandwich Theorem to show that the loss for optimizer is 0.
\subsubsection{Calibrated Cross entropy}
This method is from \cite{cao2024defense}
\begin{align}
    L_{\tilde{\psi}}(\boldsymbol{u}, y, m)=-\log \left(\tilde{\psi}_y(\boldsymbol{u})\right)-\llbracket m \neq y \rrbracket \log \left(1-\tilde{\psi}_{K+1}(\boldsymbol{u})\right)-\llbracket m=y \rrbracket \log \left(\tilde{\psi}_{K+1}(\boldsymbol{u})\right)
\end{align}
where
\begin{align}
    \tilde{\psi}_y(\boldsymbol{u})= \begin{cases}\frac{\exp \left(u_y\right)}{\sum_{y^{\prime}=1}^K \exp \left(u_{y^{\prime}}\right)}, & y \neq K+1 \\ \frac{\exp \left(u_{K+1}\right)}{\sum_{y^{\prime}=1}^{K+1} \exp \left(u_{y^{\prime}}\right)-\max _{y^{\prime} \in\{1, \cdots, K\}} \exp \left(u_{y^{\prime}}\right)}, & \text { else. }\end{cases}
\end{align}
This method is extension of \ref{subsection:ova}.

\subsection{One vs all class}\label{subsection:ova}
This method is from \cite{verma2022calibrated}.
\begin{align}
    \begin{aligned}
& \psi_{\mathrm{OvA}}\left(g_1, \ldots, g_K, g_{\perp} ; \boldsymbol{x}, y, m\right)= \\
& \quad \phi\left[g_y(\boldsymbol{x})\right]+\sum_{y^{\prime} \in \mathcal{Y}, y^{\prime} \neq y} \phi\left[-g_{y^{\prime}}(\boldsymbol{x})\right]+   \phi\left[-g_{\perp}(\boldsymbol{x})\right]+\mathbb{I}[m=y]\left(\phi\left[g_{\perp}(\boldsymbol{x})\right]-\phi\left[-g_{\perp}(\boldsymbol{x})\right]\right)
\end{aligned}
\end{align}
where
\begin{align}
    \phi[f(\boldsymbol{x})]=\log (1+\exp \{-f(\boldsymbol{x})\})
\end{align}
over optimization, $\phi[f(\boldsymbol{x})]$ would cause $f(x)$ increase and $\phi[-f(\boldsymbol{x})]$ would cause $f(x)$ decrease. In this paper, $g_y(\boldsymbol{x})$ is the output for $y-th$ neuron in network.

Proof of consistency: divide the the case into binary and then prove that for each case, the minimizer works as the same as Bayes.

Should be familiar with  "strictly proper composite loss" and " inverse link function " term. By finding those pair \textbf{("strictly proper composite loss", "inverse link function")}, we can directly get that the class probability estimate of minimizer of this loss is just inver link function.  And it's also classification calibrated.

\subsection{Methods summarized by \cite{mao2024two}}
\includegraphics[width=1\textwidth]{Figures/Screenshot 2024-02-27 at 16.55.45.png}\\
\includegraphics[width=1\textwidth]{Figures/Screenshot 2024-02-27 at 16.56.06.png}


\section{Difficulty when applies multi-class L2D methods to L2H}
\subsection{Bayes Rule}
Analogous to L2D, one of the Bayes Rule for mobile classifier and rejector are:\textcolor{red}{I think $E_{Y}[1_{e^{B}=Y}|X=x]=\eta_{\arg\max_{i}\eta_{i}(x)}(x)$. Does it equal to $\max\eta(x)$. Yes. That's why the following \ref{bayes: eb} to \ref{bayes: oringianl} are true}. 
\begin{align}
    e^{B}
    &=\arg\max_{i} \eta_{i}(x)\label{bayes: eb}\\
    r^{B}&=\mathbf{1}\left[E_{Y}[1_{M\neq Y}|X=x]<E_{Y}[1_{e^{B}\neq Y}|X=x]\right]*2-1\\
    &=\mathbf{1}[P(M\neq Y|X=x)<1-\max_{i}\eta_{i}(x)]*2-1\\
    &=\mathbf{1}\left[1-\sum_{i}\eta_{i}P(M=i|X=x)<1-\max_{i}\eta_{i}(x)]\right]*2-1\\
    &\textbf{or}\\
    &=\mathbf{1}[P(M=Y|X=x)>\max_{i}\eta_{i}(x)]*2-1\\
    &=\mathbf{1}[\sum_{i}\eta_{i}P(M=i|X=x)>\max_{i}\eta_{i}(x)]*2-1\label{bayes: oringianl}
\end{align}
If we assume $m(x)=\arg\max m_{i}(x)$, where $m_{i}$ is the output for each class in mobile NN, then the rules become:
\begin{align}
    e^{B}&=\arg\max_{i} \eta_{i}(x)\\
    r^{B}&=\mathbf{1}[E_{Y}[1_{m(x)=Y}|X=x]>\max_{i} \eta_{i}(x)]*2-1\\
    &=\mathbf{1}[E_{Y}[1_{\arg\max m_{i}(x)=Y}|X=x]>\max_{i} \eta_{i}(x)]*2-1\\
    &=\mathbf{1}[\eta_{\arg\max_{i}m_{i}(x)}(x)>\max_{i} \eta_{i}(x)]*2-1 \label{bayes: mi and etai}
\end{align}
\textcolor{red}{Then $r^{B}==-1?$, which means always reject? The result seems weird. What's the problem?}
It makes sense because when there is not cost for reject, the bayes rule would dominate when we let $m(x)=\arg\max m_{i}$. Even for deterministic case, above conclusion still holds.
\subsubsection{Quick Summary for Bayes}
When both mobile and edge are machines, the optimal for them are the same: Bayes. So it makes no sense when reject option doesn't cost (would reject forever since edge is optimal.) Posible solution:
\begin{itemize}
    \item add cost for rejecting (Then we have to handle how to interpret $\eta_{\arg\max_{i}m_{i}(x)}(x)$ and design surrogate loss for it and what's the form for rejector $r$) (Or handle with $P(M=Y|X=x)$.)
    \item edge and mobile have different input space. (For example, input for mobile is $x_1$, but for mobile is $x_1$ and $x_2$.)
    \item Refer to LWA with uninformative paper. Divide the distribution into two subsets.
\end{itemize}
\subsubsection{Legacy (Ignore them so far.)}
\textcolor{red}{are they correct?equations below} (Seems like it's incorrect.) 
\begin{align}
    e^{B}
    &=\arg\max_{i} \eta_{i}(x)\\
    r^{B}&=\mathbf{1}[\max_{i} m_{i}(x)>\max_{i} \eta_{i}(x)]*2-1\\
    &\textbf{can be formed as}\\
    &=\mathbf{1}[\max_{i} m_{i}(x)>g^{B}_{\text{reject}(x)}]*2-1\label{g_bayes:1}\\
    &\textbf{or}\\
    &=\mathbf{1}[g^{B}_{\text{reject}(x)}>\max_{i} \eta_{i}(x)]*2-1\label{g_bayes:2}
\end{align}

\subsubsection{How to design rejector}
Here, we use $g_{\text{reject}(x)}$ as reject function. $r$ is the reject rule. And if we let $m(x)=\arg\max m_i$
\begin{align}
    e^{B}
    &=\arg\max_{i} \eta_{i}(x)\\
    r^{B}&=\mathbf{1}[E_{Y}[1_{m(x)=Y}|X=x]>\max_{i} \eta_{i}(x)]*2-1\\
    &=\mathbf{1}[E_{Y}[1_{\arg\max m_{i}(x)=Y}|X=x]>\max_{i} \eta_{i}(x)]*2-1\\
    &=\mathbf{1}[\eta_{\arg\max_{i}m_{i}(x)}(x)>\max_{i} \eta_{i}(x)]*2-1\\
    &\textbf{can be formed as}\\
    &=\mathbf{1}[\eta_{\arg\max_{i}m_{i}(x)}(x)>g^{B}_{\text{reject}(x)}]*2-1\label{g_bayes:1}\\
    &\textbf{or}\\
    &=\mathbf{1}[g^{B}_{\text{reject}(x)}>\max_{i} \eta_{i}(x)]*2-1\label{g_bayes:2}
\end{align}
where $m_i$ is the output of mobile NN for $i$-th class and $g_{\text{reject}}$ is the output of the rejector. If we consider the first case \ref{g_bayes:1}.\textbf{However, the problem is how to define $g_{\text{reject}}$ and loss function, which derives to $g^{B}_{\text{reject}(x)}=\max_{i} \eta_{i}(x)$ and can work solely without knowing the output of edge during testing. Also, we need estimate $\eta_{\arg\max_{i}m_{i}(x)}(x)$ since $\eta$ is unknown to trainer}. If we consider the second case \ref{g_bayes:2}, which is the direct extension from L2D, we will have to know the edge outout before making "reject or not" decision in $r$. This case doesn't make sense since you already get the result of edge, no need to ask rejector anymore. The L2D and desired L2H framework(first case \ref{g_bayes:1}) are shown below. In L2D, the testing steps are
\begin{itemize}
    \item new $x$ comes in;
    \item calculate $m_i, i\in [K]$ and $g_{\text{reject}}$($g_{\text{reject}}$ link to $P(e=y|x=x)$, which is given by the estimate for human expert on edge.(So $P$ is known already));
    \item  comparing $g_{i}$ and $g_{\text{reject}}$, if $g_{\text{reject}}$ is the largest, reject, otherwise send choose $\arg \max_{i} g_{i}$.
\end{itemize}
If we do the similar steps for L2H:
\begin{itemize}
    \item new $x$ comes in;
    \item calculate pre-trained $m_i, i\in [K]$ and $g_{\text{reject}}$($g_{\text{reject}} \text{ optimizier should represent} \max_{i}\eta_i)$ ;
    \item  comparing $m_{i}$ and $g_{\text{reject}}$, if $g_{\text{reject}}$ is the largest, reject, otherwise send choose $\arg \max_{i} g_{i}$.
\end{itemize}

\subsubsection{Potential Solution 1 for designing rejector: Alternating optimization}
Divide the optimization into two main steps: A step update $e$ and fix $r$ and in B step update $r$ and fix $e$. Then prove that when one of $e$ and $r$ is close to bayes, the other also close to Bayes, refer to Learning to abstain from uninformative(Morgan 2023 paper). Then when update rejector $r$, the $e$ is fixed and we can estimate $P(e=Y|X=x)$ and work as L2D.

\subsubsection{Potential Solution 2 for designing rejector: multiple experts}
Assume that for K classes problem, we introduce K binary machine experts. Each expert only takes in charge of one classs, then we also have K rejectors. In this case, we dodge the difficulty that find a rejector that is equivalent to $\arg\max_{i} \eta_i$

\subsection{Proposed Loss function}
Regarding to the model I proposed in Goodnote page 43, we can design the loss function:
\begin{align}
    L&=-\ln {\frac{\exp{(e_i(x))}}{\sum_{j}\exp{(e_j(x))}}}\\
    &-\mathbf{1}_{e=y}\ln{\frac{\exp{(r_2)}}{\exp{(r_2)+\exp{(r_1)}}}}-\mathbf{1}_{m=y} \ln{\frac{\exp{(r_1)}}{\exp{(r_2)}+\exp{(r_1)}}}
\end{align}
Then the expected cost, risk, is 
\begin{align}
    \mathbb{E}_{x}\mathbb{E}_{y \mid x} L
\end{align}
The Bayes rule is optimal for any $x$. In order to derive the the Bayes rule, we can find the minimizer for each $x$.
\begin{align}
    \mathbb{E}_{y \mid x} L&=-\sum_{y \in \mathcal{Y}} \eta_y(x) \log \left(\frac{\exp \left(e_y(x)\right)}{\sum_{y^{\prime} \in \mathcal{Y} } \exp \left(e_{y^{\prime}}(x)\right)}\right)
    \\&-\mathbb{E}_{y \mid x}\mathbf{1}_{e=y}\ln{\frac{\exp{(r_2)}}{\exp{(r_2)+\exp{(r_1)}}}}
    -\mathbb{E}_{y \mid x} \mathbf{1}_{m=y} \ln{\frac{\exp{(r_1)}}{\exp{(r_2)}+\exp{(r_1)}}}
\end{align}

We can firstly find the minimzer over $e_y$. However, we notice that $e(x)$ involves in two terms, and $1_{e=y}$ is not differentiable. We choose to use "Alternating Optimization" technique, which means only optimize subset of variable at one time.

Then we divide our loss function into two part;
\begin{align}
    L_1&=-\ln {\frac{\exp{(e_i(x))}}{\sum_{j}\exp{(e_j(x))}}}\\
    L_2&=-\mathbb{E}_{y \mid x}\mathbf{1}_{e=y}\ln{\frac{\exp{(r_2)}}{\exp{(r_2)+\exp{(r_1)}}}}
    -\mathbb{E}_{y \mid x} \mathbf{1}_{m=y} \ln{\frac{\exp{(r_1)}}{\exp{(r_2)}+\exp{(r_1)}}}
\end{align}
At odd time steps, we optimize $L_1$ while at even time steps, we optimized $L_2$ and keep $e$ fixed.\\
\textcolor{red}{Not sure following step is rigorous in math or not?}\\
Since we only optimize $e$ in $L_1$, then the minimizer is the same as cross-entropy loss function
\begin{align}
    \frac{\exp{(e_i^{*}(x))}}{\sum_{j}\exp{(e_j^{*}(x))}}=\eta_i
\end{align}
Then we plug in the optimal $e(x)$ to $L_2$.
\begin{align}
    \mathbb{E}_{y \mid x} L_2&=-\mathbb{E}_{y \mid x}\mathbf{1}_{e=y}\ln{\frac{\exp{(r_2)}}{\exp{(r_2)+\exp{(r_1)}}}}
    -\mathbb{E}_{y \mid x} \mathbf{1}_{m=y} \ln{\frac{\exp{(r_1)}}{\exp{(r_2)}+\exp{(r_1)}}}\\
    &=-\max_{i}\eta_{i}\ln{\frac{\exp{(r_2)}}{\exp{(r_2)+\exp{(r_1)}}}}-\eta_{\arg\max m_{i}(x)}\ln{\frac{\exp{(r_1)}}{\exp{(r_2)}+\exp{(r_1)}}}
\end{align}
Then we take the partial derivative over $r_1$ or $r_2$ to find the minimizer. It gives the result that 
\begin{align}
    \frac{\exp{r_1}}{\exp{r_2}}=\frac{\eta_{\arg\max m_{i}(x)}}{\max_{i}\eta_{i}}
\end{align}
By comparing $r_1$ and $r_2$ to determine rejection is the same as Bayes Rule. So it's consistent loss function.
